Exoskeleton-covered soft finger with vision-based proprioception and tactile sensing

Soft robots offer significant advantages in adaptability, safety, and dexterity compared to conventional rigid-body robots. However, it is challenging to equip soft robots with accurate proprioception and tactile sensing due to their high flexibility and elasticity. In this work, we describe the development of a vision-based proprioceptive and tactile sensor for soft robots called GelFlex, which is inspired by previous GelSight sensing techniques. More specifically, we develop a novel exoskeleton-covered soft finger with embedded cameras and deep learning methods that enable high-resolution proprioceptive sensing and rich tactile sensing. To do so, we design features along the axial direction of the finger, which enable high-resolution proprioceptive sensing, and incorporate a reflective ink coating on the surface of the finger to enable rich tactile sensing. We design a highly underactuated exoskeleton with a tendon-driven mechanism to actuate the finger. Finally, we assemble 2 of the fingers together to form a robotic gripper and successfully perform a bar stock classification task, which requires both shape and tactile information. We train neural networks for proprioception and shape (box versus cylinder) classification using data from the embedded sensors. The proprioception CNN had over 99\% accuracy on our testing set (all six joint angles were within 1 degree of error) and had an average accumulative distance error of 0.77 mm during live testing, which is better than human finger proprioception. These proposed techniques offer soft robots the high-level ability to simultaneously perceive their proprioceptive state and peripheral environment, providing potential solutions for soft robots to solve everyday manipulation tasks. We believe the methods developed in this work can be widely applied to different designs and applications.

==> networks.tex <==
% For degree regression
\paragraph{Network Architecture.} Given that the inputs are 2D images, we leverage the fully convolutional neural network~\ref{Long2015fcn}. The architecture of the network we use is a sequential model of 4 convolutional layers with batch normalization and ReLU. We feed the extracted feature into a convolutional layer with sigmoid activation function to obtain the angle vector (see Fig~\ref{fig:deg_net}). 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\linewidth]{Figure/deg_net.png}
    \vspace{-4pt}
	\caption{experiment setup}
	\label{fig:deg_net}
\end{figure}


\paragraph{Data Pre-processing & Augmentation.} 
Noticing that the groundtruth angles have significantly different variance, we normalize the groundtruth angles by substracting the mean values and dividing by the standard deviations to make the individual data points comparable. The mean values and standard deviations are estimated by only using data from the training set. During the test procedure, we rescale the predicted angle by multiplying the standard deviations and adding the mean values.
We add gaussian noise with zero mean to the groundtruth angles to simulate the possible perturbation in real world scenario. The variance of the noise is set to 1e-3 to ensure that the groundtruth data will not be overwhelmed by the noise.
To improve the robustness of the model to illumination changes, we augment the image data by randomly changing the contrast and saturation of the images. 

% For size estimation
\paragraph{Network Architecture.} We consider 3 architectures to incorporate the class information (i.e., class label) into the size estimation process: \emph{Multiple Layer Perceptron (MLP)} model 
%not sure whether we should cite something here
, \emph{Two-path MLP} model and our proposed approach \emph{MLP with Neural Incorporator}.  
For the MLP model, we view the class label as an additional channel of input, so the input of the model is the concatenation of predicted angles and class label (see Fig~\ref{fig:size_net_1}). The model is simple but sets a baseline to assess the performance of other methods.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\linewidth]{Figure/size_net_1.png}
    \vspace{-4pt}
	\caption{experiment setup}
	\label{fig:size_net_1}
\end{figure}

The intuition behind the Two-path MLP model (see Fig~\ref{fig:size_net_2}) is that the class label information and the angle information come from data source, so it would be better to use a heterogeneous architecture that processes color and depth information differently, retaining the native structure of each data source. We use two paths of MLP to separately process the predicted class label and angles, and then merge them by concatenation in the latent space to extract the feature. The feature is then fed into a final MLP to perform the size estimation.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\linewidth]{Figure/size_net_2.png}
    \vspace{-4pt}
	\caption{experiment setup}
	\label{fig:size_net_2}
\end{figure}

In order to obtain a better feature representation, we propose the Neural Incorporator model to facilitate the feature extraction process in Two-path MLP model. Inspired by~\ref{Park2019spade}, we use the feature learned from the class label $\beta, \gamma$ to normalize the feature learned from the predicted angles $f$ (see Fig~\ref{fig:size_net_3}),
\begin{equation}
    \hat{f} = f*(1 + \gamma) + \beta
\end{equation}{}
The normalized feature $\hat{f}$ is then fed into a final MLP to perform the size estimation.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\linewidth]{Figure/size_net_3.png}
    \vspace{-4pt}
	\caption{experiment setup}
	\label{fig:size_net_3}
\end{figure}

\paragraph{Training Procedure.} 
We use Adam optimizer to train the degree regression network for 50 epochs. The learning rate is set to 1e-4 at the beginning, and gradually decreases to 1e-5 as the training epoch increases. 
We use the same setting to train the size estimation network except that the initial learning rate is set to 1e-3.

% Experiment section
% \paragraph{Evaluation.} We evaluate the quality of the regression on XXX test images per object. The error reported is the RMSE (Root Mean Squared Error) between the actual and predicted heightmaps w.r.t. to the size of the contact patch. To first order, we see that the RMSE decreases by adding more training data and that the average reconstruction accuracy reaches 0.1mm on the test data with only 500 datapoints and 0.060±0.016mm using 2000 datapoints. 
% Table I shows the average RMSE (mm) of the heightmap reconstruction on novel shapes by a cross-validation approach. For each training object, we remove it entirely from the training set, train a CNN with 2000 datapoints, and evaluate it both on the whole test set and just on the images from the removed object. Even for hold-out objects, the reconstruction accuracy is on the order of 0.1mm. We observe experimentally that objects like semicone1 or hollow that have unique geometric features, such as edges and holes, are more important to the training set. Smaller objects that leave a more reliable imprint on the sensor are also more informative for the training set. 
% Finally, Fig. 3 shows three examples of how we recover the local shape of novel complex objects. Results indicate that the map built to translate tactile imprints to heightmaps is accurate at recovering the local geometry of objects and can be extended to reconstruct their global shapes.
